The life cycle of stars and their planets from the high energy perspective

One of the key research themes identified by the Astro2020 decadal survey is Worlds and Suns in Context. The Advanced X-ray Imaging Satellite (AXIS) is a proposed NASA APEX mission that will become the prime high-energy instrument for studying star-planet connections from birth to death. This work explores the major advances in this broad domain of research that will be enabled by the AXIS mission, through X-ray observations of stars in clusters spanning a broad range of ages, flaring M-dwarf stars known to host exoplanets, and young stars exhibiting accretion interactions with their protoplanetary disks. In addition, we explore the ability of AXIS to use planetary nebulae, white dwarfs, and the Solar System to constrain important physical processes from the microscopic (e.g., charge exchange) to the macroscopic (e.g., stellar wind interactions with the surrounding interstellar medium).

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}
